A study of a contact binary system NSVS 2983201

Here we present the observations and the first light curve analysis of the short-period variable star NSVS 2983201. Using the light curve numerical modeling we find the best fitting model to be of shallow (ff=10%) contact binary configuration of mass ratio q=0.36. The light curve of the system experiences the O'Connell effect, which led to identifying a large circumpolar starspot. With a careful multi-cases analysis we search for the physical parameters of the system. We find the results obtained with the different methods to be close, but not overlapping. This system will be scheduled for the further monitoring.

==> biblio.tex <==
\bibitem[Latkovi{\'c}, {\v{C}}eki, and Lazarevi{\'c}(2021)]{2021ApJS..254...10L}Latkovi{\'c}, O., {\v{C}}eki, A., and Lazarevi{\'c}, S.: 2021, {\it The Astrophysical Journal Supplement Series} {\bf 254}, 10. doi:10.3847/1538-4365/abeb23.
\bibitem[Lindegren \emph{et al.}(2021)]{2021A&A...649A...4L}Lindegren, L., Bastian, U., Biermann, M., Bombrun, A., de Torres, A., Gerlach, E., and, ...: 2021, {\it Astronomy and Astrophysics} {\bf 649}, A4. doi:10.1051/0004-6361/202039653.
\bibitem[Ren \emph{et al.}(2021)]{2021ApJ...911L..20R}Ren, F., Chen, X., Zhang, H., de Grijs, R., Deng, L., and Huang, Y.: 2021, {\it The Astrophysical Journal} {\bf 911}, L20. doi:10.3847/2041-8213/abf359.
\bibitem[Li, Liu, and Zhu(2020)]{2020PASJ...72..103L}Li, X.-Z., Liu, L., and Zhu, L.-Y.: 2020, {\it Publications of the Astronomical Society of Japan} {\bf 72}, 103. doi:10.1093/pasj/psaa104.
\bibitem[Debski(2020)]{2020CoSka..50..490D}Debski, B.: 2020, {\it Contributions of the Astronomical Observatory Skalnate Pleso} {\bf 50}, 490. doi:10.31577/caosp.2020.50.2.490.
\bibitem[Debski(2019)]{2019CoSka..49..258D}Debski, B.: 2019, {\it Contributions of the Astronomical Observatory Skalnate Pleso} {\bf 49}, 258.
\bibitem[Samec \emph{et al.}(2018)]{2018RNAAS...2...13S}Samec, R., Caton, D., Robb, R., and Faulkner, D.R.: 2018, {\it Research Notes of the American Astronomical Society} {\bf 2}, 13. doi:10.3847/2515-5172/aaa7ed.
\bibitem[Debski and Zola(2017)]{2017IAUS..325..274D}Debski, B. and Zola, S.: 2017, {\it Astroinformatics} {\bf 325}, 274. doi:10.1017/S1743921316013077.
\bibitem[Zola \emph{et al.}(2017)]{2017MNRAS.466.2488Z}Zola, S., Baran, A., Debski, B., and Jableka, D.: 2017, {\it Monthly Notices of the Royal Astronomical Society} {\bf 466}, 2488. doi:10.1093/mnras/stw3138.
\bibitem[Debski, Zola, and Baran(2015)]{2015ASPC..496..293D}Debski, B., Zola, S., and Baran, A.: 2015, {\it Living Together: Planets, Host Stars and Binaries} {\bf 496}, 293.
\bibitem[Debski(2015)]{2015salt.confE..64D}Debski, B.: 2015, {\it SALT Science Conference 2015 (SSC2015)}, 64.
\bibitem[Debski(2015)]{2015salt.confE..65D}Debski, B.: 2015, {\it SALT Science Conference 2015 (SSC2015)}, 65.
\bibitem[Debski and Zo{\l}a(2014)]{2014bsee.confP..42D}Debski, B. and Zo{\l}a, S.: 2014, {\it Binary Systems, their Evolution and Environments}, P4-2.
\bibitem[Debski, Baran, and Zola(2014)]{2014CoSka..43..427D}Debski, B., Baran, A., and Zola, S.: 2014, {\it Contributions of the Astronomical Observatory Skalnate Pleso} {\bf 43}, 427.
\bibitem[Pecaut and Mamajek(2013)]{2013ApJS..208....9P}Pecaut, M.J. and Mamajek, E.E.: 2013, {\it The Astrophysical Journal Supplement Series} {\bf 208}, 9. doi:10.1088/0067-0049/208/1/9.
\bibitem[Claret, Hauschildt, and Witte(2013)]{2013A&A...552A..16C}Claret, A., Hauschildt, P.H., and Witte, S.: 2013, {\it Astronomy and Astrophysics} {\bf 552}, A16. doi:10.1051/0004-6361/201220942.
\bibitem[Brown \emph{et al.}(2011)]{2011AJ....142..112B}Brown, T.M., Latham, D.W., Everett, M.E., and Esquerdo, G.A.: 2011, {\it The Astronomical Journal} {\bf 142}, 112. doi:10.1088/0004-6256/142/4/112.
\bibitem[Schlafly and Finkbeiner(2011)]{2011ApJ...737..103S}Schlafly, E.F. and Finkbeiner, D.P.: 2011, {\it The Astrophysical Journal} {\bf 737}, 103. doi:10.1088/0004-637X/737/2/103.
\bibitem[Claret and Bloemen(2011)]{2011A&A...529A..75C}Claret, A. and Bloemen, S.: 2011, {\it Astronomy and Astrophysics} {\bf 529}, A75. doi:10.1051/0004-6361/201116451.
\bibitem[Pr{\v{s}}a \emph{et al.}(2011)]{2011AJ....141...83P}Pr{\v{s}}a, A., Batalha, N., Slawson, R.W., Doyle, L.R., Welsh, W.F., Orosz, J.A., and, ...: 2011, {\it The Astronomical Journal} {\bf 141}, 83. doi:10.1088/0004-6256/141/3/83.
\bibitem[Zola \emph{et al.}(2010)]{2010MNRAS.408..464Z}Zola, S., Gazeas, K., Kreiner, J.M., Ogloza, W., Siwak, M., Koziel-Wierzbowska, D., and, ...: 2010, {\it Monthly Notices of the Royal Astronomical Society} {\bf 408}, 464. doi:10.1111/j.1365-2966.2010.17129.x.
\bibitem[Gazeas and St{\c{e}}pie{\'n}(2008)]{2008MNRAS.390.1577G}Gazeas, K. and St{\c{e}}pie{\'n}, K.: 2008, {\it Monthly Notices of the Royal Astronomical Society} {\bf 390}, 1577. doi:10.1111/j.1365-2966.2008.13844.x.
\bibitem[Pribulla and Rucinski(2006)]{2006AJ....131.2986P}Pribulla, T. and Rucinski, S.M.: 2006, {\it The Astronomical Journal} {\bf 131}, 2986. doi:10.1086/503871.
\bibitem[Jester \emph{et al.}(2005)]{2005AJ....130..873J}Jester, S., Schneider, D.P., Richards, G.T., Green, R.F., Schmidt, M., Hall, P.B., and, ...: 2005, {\it The Astronomical Journal} {\bf 130}, 873. doi:10.1086/432466.
\bibitem[Csizmadia and Klagyivik(2004)]{2004A&A...426.1001C}Csizmadia, S. and Klagyivik, P.: 2004, {\it Astronomy and Astrophysics} {\bf 426}, 1001. doi:10.1051/0004-6361:20040430.
\bibitem[Rucinski(2004)]{2004NewAR..48..703R}Rucinski, S.M.: 2004, {\it New Astronomy Reviews} {\bf 48}, 703. doi:10.1016/j.newar.2004.03.005.
\bibitem[Pribulla, Kreiner, and Tremko(2003)]{2003CoSka..33...38P}Pribulla, T., Kreiner, J.M., and Tremko, J.: 2003, {\it Contributions of the Astronomical Observatory Skalnate Pleso} {\bf 33}, 38.
\bibitem[Webbink(2003)]{2003ASPC..293...76W}Webbink, R.F.: 2003, {\it 3D Stellar Evolution} {\bf 293}, 76.
\bibitem[Bonnarel \emph{et al.}(2000)]{2000A&AS..143...33B}Bonnarel, F., Fernique, P., Bienaym{\'e}, O., Egret, D., Genova, F., Louys, M., and, ...: 2000, {\it Astronomy and Astrophysics Supplement Series} {\bf 143}, 33. doi:10.1051/aas:2000331.
\bibitem[Hendry and Mochnacki(2000)]{2000ApJ...531..467H}Hendry, P.D. and Mochnacki, S.W.: 2000, {\it The Astrophysical Journal} {\bf 531}, 467. doi:10.1086/308427.
\bibitem[Lucy(1976)]{1976ApJ...205..208L}Lucy, L.B.: 1976, {\it The Astrophysical Journal} {\bf 205}, 208. doi:10.1086/154265.
\bibitem[Flannery(1976)]{1976ApJ...205..217F}Flannery, B.P.: 1976, {\it The Astrophysical Journal} {\bf 205}, 217. doi:10.1086/154266.
\bibitem[Mullan(1975)]{1975ApJ...198..563M}Mullan, D.J.: 1975, {\it The Astrophysical Journal} {\bf 198}, 563. doi:10.1086/153635.
\bibitem[Lucy(1968)]{1968ApJ...153..877L}Lucy, L.B.: 1968, {\it The Astrophysical Journal} {\bf 153}, 877. doi:10.1086/149712.
\bibitem[Lucy(1968)]{1968ApJ...151.1123L}Lucy, L.B.: 1968, {\it The Astrophysical Journal} {\bf 151}, 1123. doi:10.1086/149510.
\bibitem[Eggen(1967)]{1967MmRAS..70..111E}Eggen, O.J.: 1967, {\it Memoirs of the Royal Astronomical Society} {\bf 70}, 111.
\bibitem[O'Connell(1951)]{1951PRCO....2...85O}O'Connell, D.J.K.: 1951, {\it Publications of the Riverview College Observatory} {\bf 2}, 85.
\bibitem[Muller and Kempf(1903)]{1903ApJ....17..201M}Muller, G. and Kempf, P.: 1903, {\it The Astrophysical Journal} {\bf 17}, 201. doi:10.1086/141011.
